Risk Minimization in Structured Prediction using Orbit Loss

We introduce a new surrogate loss function called orbit loss in the structured prediction framework, which has good theoretical and practical advantages. While the orbit loss is not convex, it has a simple analytical gradient and a simple perceptron-like learning rule. We analyze the new loss theoretically and state a PAC-Bayesian generalization bound. We also prove that the new loss is consistent in the strong sense; namely, the risk achieved by the set of the trained parameters approaches the infimum risk achievable by any linear decoder over the given features. Methods that are aimed at risk minimization, such as the structured ramp loss, the structured probit loss and the direct loss minimization require at least two inference operations per training iteration. In this sense, the orbit loss is more efficient as it requires only one inference operation per training iteration, while yields similar performance. We conclude the paper with an empirical comparison of the proposed loss function to the structured hinge loss, the structured ramp loss, the structured probit loss and the direct loss minimization method on several benchmark datasets and tasks.

==> gmm.tex <==
\chapter{Discriminative Training for Generative Models}\label{ch:generative_model}

In this chapter we propose our discriminative method for generative model and demonstrate it on continuous density Hidden Markov Models (CD-HMMs). We suggest an alternative training method to the perceptron and large margin approaches as suggested in \citep{Collins2002} and \citep{FeiSha09} that present online learning algorithms for CD-HMMs. The target task is an automatic speech recognition task (ASR) and the emission densities are computed from Gaussian Mixture Models (GMMs).

\input{ch-generative/section-gmm}
Recall that in ASR we seek to model the joint distributions $\mathcal{P}(\vx, \vy)$ over sequences of hidden (phonetic) states  $\vy = \{y_1, y_2, \dots , y_T \}$ and acoustic observations or feature vectors $\vx = \{\vx_1, \vx_2, \dots, \vx_T \}$. In Continuous Density Hidden Markov Models (CD-HMMs), the distribution is parameterized with an initial state distribution $\mathcal{P}(y_1)$, state transition probabilities $\mathcal{P}(y_{t+1}|y_t)$, and emission densities $\mathcal{P}(\vx_{t}|y_t)$. Concretely,
\begin{equation}\label{eq:distribution}
	\mathcal{P}(\vx|y) = \mathcal{P}(y_1)\prod_{t=1}^{T-1}\mathcal{P}(y_{t+1}|y_t)\prod_{t=1}^{T}\mathcal{P}(\vx_{t}|y_t)
\end{equation}
 For each state $y$ and mixture component $c$, we denote the mean vector by $\mu_{yc}$ and the covariance matrix by $\Sigma_{yc}$. Using this notation, the emission densities are given by:
\begin{equation}\label{abstract_gmm_score}
	\mathcal{P}(\vx_{t}|y_t) = \sum_c\mathcal{P}(c|y)\mathcal{N}(\mu_{yc},\Sigma_{yc}) 
\end{equation}
where $\mathcal{N}(\mu,\Sigma)$ denotes a multivariate Gaussian and $\mathcal{P}(c|y)$ denotes mixture weights.

The discriminant function over observation and state transition sequences is defined as follows:
\begin{equation}
	\mathcal{D}(\vx, \vy) = \log\mathcal{P}(y_1) + \sum_{t=1}^{T-1}\log\mathcal{P}(y_{t+1}|y_{t}) + \sum_{t}\log\mathcal{P}(\vx_{t}|y_t)
\end{equation}
which is simply the logarithm of the joint distribution in \eqref{eq:distribution}. Let $\vy$ denote the correct transcription
of the observation sequence $\vx$. For correct recognition, we require that 
\begin{equation}
	\forall\vy' \neq \vy, \mathcal{D}(\vx, \vy) > \mathcal{D}(\vx, \vy')
\end{equation}
Denote $\hat{\vy}$ as the the optimal decoding:
\begin{equation}
	\hat{\vy} = \argmax_{\vy'}\mathcal{D}(\vx, \vy'),
\end{equation}
which can be efficiently computed by the Viterbi algorithm.
Let $\Theta$ denote the parameters of the emission model --- GMM in our case. Note that the HMM parameters are not updated in this work and in the mentioned papers.
Let $(\vx_n, \vy_n)$
denote the acoustic observations and ground truth hidden state
transcriptions of the $n$th training utterance. 

The update rule for the perceptron is defined as follows:
\begin{equation}\label{eq:gmm_perceptron_update_rule}
	\Theta \leftarrow \Theta + \eta\frac{\partial}{\partial\Theta}\big[\mathcal{D}(\vx_n, \vy_n) - \mathcal{D}(\vx_n, \hat{\vy})\big]
\end{equation}

Exactly like in the perceptron case we use $\hat{\vy}$ for inference. Thus, the update rule for \emph{orbit loss} is:
\begin{equation}
	\Theta \leftarrow \Theta + \eta\ell(\vy_n,\hat{\vy})\frac{\partial}{\partial\Theta}\big[\mathcal{D}(\vx_n, \vy_n) - \mathcal{D}(\vx_n, \hat{\vy})\big]
\end{equation} 
where $\ell(\vy_n,\hat{\vy})$ is the cost for mispredicting $\hat{\vy}$ while the ground truth sequence is $\vy_n$.

\section{Conclusion}
In this chapter we suggested a derivation for the orbit loss for generative models, thus, offering a comprehensive solution for both discriminative and generative models. We will examine the performance of our approach in its generative form in chapter \ref{ch:experiments}.

==> section-gmm.tex <==
\subsection{Gaussian Mixture Model (GMM)}
The \textit{Gaussian Mixture Model} is a probabilistic model for representing the presence of subpopulations within an overall population, where each subpopulation can be described with gaussian properties. From a probabilistic perspective, if our label set $\Yc$ can be represented as a GMM then $\forall i: \vy_i \in \Yc ,\ \vy_i = \{ \{c_j\}_{j=1}^t: \ c_j = \{\mu, \Sigma, \pi\} \}$, where $\mu$ represents the component's mean, $\Sigma$ the component's co-variance and $\pi$ the component's weight. It should be noted that given an instance $\vx$ the identity of the sub-population $m_j$ is not required, whereas the identity of the overall population is, i.e. its label $\vy_i$.

The inference rule for a model based exclusively on GMM is:
\[ \hat{\vy} = \arg\max_{\vy \in \Yc} \sum_{c=1}^k\pi_{yc} \Nc(\mu_{yc}, \Sigma_{yc}), \]
that is, we return the label with the associated highest weighted score. 

The GMM model is appropriate for both supervised and unsupervised tasks and offers an external complexity representation level that can be highly beneficial for complex tasks. Learning tasks like \textit{phoneme alignment} use GMM to produce superior performance.

As mentioned previously, training and optimizing a generative model using a discriminative approach is quite challenging. Consider the GMM case, for example, where each mixture component in this model is parametrized using three parameters: mean, covariance and weight. Each parameter has its own constraints and applying an update rule according to the discriminative approach on each parameter separately can either violate the constrains of the other parameters or require the careful tuning of multiple learning rates in order to succeed. 

Alternatively, \citet{ShaSa09} introduced matrix representation for a mixture component’s parameters $\{\mu_{yc}, \Sigma_{yc}, \pi_{yc}\}$ as elements of the following matrix: 
$$ 
\Phi_{yc} = 
\left[ 
  \begin{tabular}{cc}
  $\Sigma_{yc}^{-1}$  & $-\Sigma_{yc}^{-1}\mu_{yc}$ \\
  $-\mu_{yc}^{\top}\Sigma_{yc}^{-1}$  & $\mu_{yc}^{\top}\Sigma_{yc}^{-1}\mu_{yc} +\pi_{yc}$
    \end{tabular}
\right]
$$
This representation allows applying update rules according to  discriminative algorithms, such as \textit{perceptron, large-margin} and, of course, \textit{orbit loss} without violating any constrains or special tuning nor treatment.

In order to use the this representation it is required to modify the original form of instances as following:
$$ \vz_t = \left[ 
  \begin{tabular}{c}
		$\vx_t$ \\
		1
    \end{tabular}
\right]
$$

We replace \eqref{abstract_gmm_score} with the following:
\begin{equation}
	\mathcal{P}(\vx_{t}|y_t) = \log \sum_{c}e^{-\vz_t^\top\Phi_{yc}\vz_t}
\end{equation}
Though not mandatory, we use this representation in chapter \ref{ch:generative_model} to present the necessary derivation for the orbit loss in order to apply it on generative models.

